Cross-device Federated Learning for Mobile Health Diagnostics: A First Study on COVID-19 Detection

Federated learning (FL) aided health diagnostic models can incorporate data from a large number of personal edge devices (e.g., mobile phones) while keeping the data local to the originating devices, largely ensuring privacy. However, such a cross-device FL approach for health diagnostics still imposes many challenges due to both local data imbalance (as extreme as local data consists of a single disease class) and global data imbalance (the disease prevalence is generally low in a population). Since the federated server has no access to data distribution information, it is not trivial to solve the imbalance issue towards an unbiased model. In this paper, we propose FedLoss, a novel cross-device FL framework for health diagnostics. Here the federated server averages the models trained on edge devices according to the predictive loss on the local data, rather than using only the number of samples as weights. As the predictive loss better quantifies the data distribution at a device, FedLoss alleviates the impact of data imbalance. Through a real-world dataset on respiratory sound and symptom-based COVID-$19$ detection task, we validate the superiority of FedLoss. It achieves competitive COVID-$19$ detection performance compared to a centralised model with an AUC-ROC of $79\%$. It also outperforms the state-of-the-art FL baselines in sensitivity and convergence speed. Our work not only demonstrates the promise of federated COVID-$19$ detection but also paves the way to a plethora of mobile health model development in a privacy-preserving fashion.

==> 0_Intro_1.tex <==
\section{Introduction}
The popularity of mobile devices and the advance in artificial intelligence empowers smart personal health sensing and computing~\cite{steinhubl2015emerging}. However,  the promise is inseparable from large-scale data, which is not easy to collect due to privacy concerns.  Federated learning (FL), which enables collaborative model training across a variety of clients without raw data disclosure
~\cite{nguyen2021federated,nguyen2022federated}, opens a new way for privacy-preserving model development. \tx{Comment}
%This can further encourage a larger fraction of the population to contribute to model developments in a privacy-preserving fashion~\cite{sadilek2021privacy}.

% The popularity of mobile devices and the advance of artificial intelligence empowers smart personal health sensing and computing~\cite{steinhubl2015emerging}. Despite the great promise, developing high-performance deep learning-driven health diagnostic models, as well known, is inseparable from large-scale data. Nevertheless, due to privacy concerns, i.e., the risk of sharing sensitive health information and digital signals, gathering data in a centralised database is not always available and thus hinders model development.   To address this problem, federated learning (FL) recently has been investigated to enable collaborative model training across a variety of clients without raw data disclosure~\cite{nguyen2021federated,nguyen2022federated}. This can further encourage a larger fraction of the population to contribute to model developments in a privacy-preserving fashion~\cite{sadilek2021privacy}.

In this paper, we aim to verify the feasibility of federated learning in developing a personal disease detection model from individuals' health signals. 
As displayed in Fig.~\ref{fig:fed}, such a cross-individual federated system is composed of many clients (mobile users) and a server. On the client side,  digital signals are recorded and  disease labels are annotated by individuals for local model training, under the coordination of the server. The server will then update the global model by aggregating the gradients shared by clients and send the new model back to clients for the next round of learning. After many iterations, it will finally end up with a converged global model which can be deployed to uninvolved individuals for disease diagnosis. 

\ag{I understand the meaning of cross-individual FL. But, may be this can also be called as cross-device, as the data of an individual is from a single device? In that case it'll be more inline with the literature.

Does the ML has anything to do with individuals? In other words, if one randomly shuffles the samples in between individuals will the analysis remain the same?}
\tx{Cross-device is acceptable, but I used cross-individually for two reasons: 1) disease is an individual attribute. One can have many devices but only one type of disease. 2) we don't handle the device heterogeneity in terms of memory etc.} 

 \begin{figure}[t]
\centering
\vspace{-15pt}
\includegraphics[width=0.4\textwidth]{figure/federated.png}
\vspace{-10pt}
\caption{Federated learning system for mobile health diagnosis. \ag{I usually do superscripts with brackets like $D^{(2)}$ to avoid confusions. The trained model can also be used to predict on the future samples from the nodes that participated in training? So, it does not need to be new users?}}\label{fig:fed}
\end{figure}


Challenges of this cross-individual FL task span several aspects.  First, each client only holds limited training data that are most likely from a single class (i.e., a person's health status will not change dramatically in a short period). Consequently, the client model could be over-fitted and biased towards its class, and furthermore, if the local training and the global updating are not coordinated properly, the global model can hardly converge. \ag{Didn't get this. What do you mean hardly converge and the reason is unclear to me.} Besides, the global data distribution is usually imbalanced (i.e., there are far more healthy than unhealthy users in real life). Because of the invisibility of local labels, the server-side aggregation\ag{Unclear. say something like as the server does not have access to private disease labels the aggregation step may introduce unwanted bias towards the majority class in the system.} may also cause a global model biased towards the majority healthy population, yielding a high false negative rate. Those two challenges are known as \emph{data statistical heterogeneity}, while another  bottleneck hindering the model performance is the clients' \emph{participation availability}. Constrained by resource and power, not all users can participate in training at any time, and hence  fewer rounds of local training and communication is highly desired during the  process. 
\ag{The resource challenge comes out of the blue.

May be the following can be a flow for the introduction. Mobile phones can capture individual health signals -- Though the signal is useful it may contain sensitive information and thus cannot be just aggregated as raw data -- And the sensing happens continually so it generates huge amount of data sending which will incur huge cost.

Then say FL is usually a solution to these. It has been popular in health application as well, but most consider cross-silo setup on clinical data. However, to build population-level scalable systems one needs to use the smart edge device based cross-device FL. Then say its advantages: low cost, scalable, private. But challenges are i) Class imbalance, ii) most devices have single class, iii) resources. Is there any audio related challenge for FL?

Introduce the data: We consider Covid-19 where the disease state is transient, i.e., a person changes her state from susceptible to infected and finally to recover within a few days. Our data consists of audio signals, .... at temporal snapshots where the data can be processed to predict the state.} \tx{Good Suggestion! I am rephrasing now}

To address the aforementioned challenges, in this paper, we propose a novel algorithm, namely \emph{FedLoss}, for effective and efficient federated model training. The novelty of \emph{FedLoss} lies in its adaptive model aggregation: Only a small number of clients are required to train the model synchronously in each round, and their models are aggregated according to adaptive weights guided by the predictive loss on the corresponding data.

% \tx{To be shorten} To address the aforementioned challenges, in this paper, we propose a novel algorithm, namely \emph{FedLoss}, for effective and efficient collaborative model training.
% To handle the data statistical heterogeneity, \emph{FedLoss} is devised to launch relatively fewer local training iterations and more frequent global updating to improve model generalisation. More importantly, differing from the standard federated aggregation in \emph{FedAvg}~\cite{mcmahan2017communication,li2020federated,gao2022end,feng2022federated}, the simple average operation is replaced by our dynamically weighted aggregation with the weight proportionally to the loss of local data in the corresponding client. As it is more difficult to correctly predict the minority unhealthy users, particularly at the begin of learning, they will have larger weights when their models are aggregated into the new global model, alleviating the impact of global data imbalance. Those above designs, additionally, allow partly participation. Specifically, only a small number of clients are required to train model synchronously in our algorithm.


We validate our proposed \emph{FedLoss} via a COVID-19 detection task, where audio and symptoms
are leveraged to screen COVID-19 positive users.
A dataset covering about 3,000 users with COVID-19 test status is used for experiments. With the assumption that all clients can keep the data until the global model gets converged,  our \emph{FedLoss} outperforms baselines by 30\% higher sensitivity and up to 4× speedup in convergence to the target ROC-AUC.  
Under the setting that clients only keep the data for a short period, \emph{FedLoss} still achieves competitive performance against the centralised training model with an AUC-ROC of 79\%. Those results demonstrate the promise of training a COVID-19 detection model, and also models for other similar healthcare tasks,  without centralising personal data. 


%large scale users in a privacy-preserving way.

==> 2_Data.tex <==
% \section{Data and COVID-19 Detection Model}
% \jh{this section is not a focus of this work, neither very general, hence suggest to move it to later part, either as an additional subsection in method section, eg `FedLoss for COVID-19 Detection', or move it to experiment}
% This section presents a description of the data and the COVID-19 detection model design from the acquired data.  
\begin{figure}[t]
  \centering
  \subfigure[Demographics.]{
  \includegraphics[width=0.225\textwidth]{figure/demo.png}}
  \vspace{-6pt}
  \subfigure[Symptoms distribution.]{
  \includegraphics[width=0.235\textwidth]{figure/symp.png}}
  \subfigure[User data amount.]{
  \includegraphics[width=0.215\textwidth]{figure/hist.png}}
  \vspace{-10pt}
  \subfigure[Monthly Data amount.]{
  \includegraphics[width=0.25\textwidth]{figure/num_date.png}}
  \caption{Data statistics overview. 
  %(a) Negative and positive group present similar demographic distribution. (b) 52.1\% and 86.5\% of the tested negative and positive users are symptomatic respectively, but their reported symptoms show different patterns. (c) Data amount per user. (D) Data account per month.
  }
  \label{fig:data}
   \vspace{-10pt}
\end{figure}  

\vspace{-8pt}
\subsection{Data Details}
\vspace{-5pt}
A mobile application named \emph{COVID-19 Sounds}\footnote{\url{www.covid-19-sounds.org}} has been launched to the public to collect data from individuals. Each user was assigned a unique anonymous ID when they registered the application by filling out a basic demographic and medical history questionnaire. Every two days the application reminds the user to record the data, including symptoms, three audio recordings (i.e., breathing, coughing, and voice), and the COVID-19 testing status~\cite{han2021exploring}. 

As of April 2021, a total number of 36,116 participants registered the application~\cite{xia2021covid}. In this paper, we select  English-spoken users with either COVID-19 tested positive or negative results and high-quality audio recordings,  for experiments~\cite{xia2021covid}. Consequently,  482 tested positive users and 
 2,478 tested negative users with a total of xx samples included. An overall review of the statistics of the data is illustrated in Fig.~\ref{fig:data}. The crowded-sourced data is representative with a wide demographic coverage (refer to Fig.~\ref{fig:data}(a)). But this data is also very heterogeneous: more negative than positive users, many asymptomatic positive users while a great proportion of the negative users reported respiratory disease-related symptoms (see Fig.~\ref{fig:data}(b)), user data sparsity with over 70\% of users only recording one sample, and the slow data accumulation procession spanning around 1 year. Such data heterogeneity poses extra challenges to federate learning systems for COVID-19 detection. 



\vspace{-5pt}
 \subsection{Backbone COVID-19 Detection Model}
 \vspace{-2pt}
Following the previous work~\cite{xia2021covid,han2022sounds}, a VGG framework is adapted to extract acoustic features from the spectrogram of audio samples. Additionally, Jing \emph{et al.} found\jh{reported or observed} that confusing\jh{fusing you mean?} the symptoms and acoustic features in an early stage of the classifier can achieve better COVID-19 detection performance than using a single type of feature. Inspired by those prior works, we propose a multi-modal deep learning model to predict COVID-19 status from audio and symptoms jointly, as illustrated in Fig.~\ref{fig:model}. Symptoms are represented by a multi-hot vector, which is concatenated with the dense feature from VGGish network outputs. The confused feature will then be fed into multi-layer fully connected networks for classification.  \emph{Softmax} is finally used to output the probabilities of the positive and the negative class.


\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{figure/model.png}
\caption{\label{fig:model} COVID-19 detection from symptoms and sounds.}
 \vspace{-10pt}
\end{figure}


 


